On the Sustainability of AI Inferences in the Edge

The proliferation of the Internet of Things (IoT) and its cutting-edge AI-enabled applications (e.g., autonomous vehicles and smart industries) combine two paradigms: data-driven systems and their deployment on the edge. Usually, edge devices perform inferences to support latency-critical applications. In addition to the performance of these resource-constrained edge devices, their energy usage is a critical factor in adopting and deploying edge applications. Examples of such devices include Raspberry Pi (RPi), Intel Neural Compute Stick (INCS), NVIDIA Jetson nano (NJn), and Google Coral USB (GCU). Despite their adoption in edge deployment for AI inferences, there is no study on their performance and energy usage for informed decision-making on the device and model selection to meet the demands of applications. This study fills the gap by rigorously characterizing the performance of traditional, neural networks, and large language models on the above-edge devices. Specifically, we analyze trade-offs among model F1 score, inference time, inference power, and memory usage. Hardware and framework optimization, along with external parameter tuning of AI models, can balance between model performance and resource usage to realize practical edge AI deployments.

==> input_batch_size_comparison.tex <==
\section{Research Question}
\textit{How do variations in input size, batch size, and token window length impact inference time, energy consumption, and model accuracy when transformer-based and deep learning models are deployed on edge devices?}

\section{Motivation}
The deployment of deep neural network models on edge devices has enabled a wide range of applications—from smart home assistants to autonomous systems. However, these devices are inherently limited by constrained computational resources and strict energy budgets, making energy-efficient inference an essential challenge.

Recent work has shown that key workload parameters—namely, input size, batch size, and token window length—profoundly impact both inference latency and energy consumption. For example, larger input sizes can provide richer contextual information and improve accuracy, yet they lead to a quadratic increase in computational complexity in transformer-based models due to the self-attention mechanism \cite{zhang2024edge}. Similarly, while increasing the batch size can boost throughput via improved parallelism, it may also impose excessive memory pressure and elevate energy usage if the device’s capacity is exceeded \cite{shi2022multi}. In addition, extending the token window length enhances context retention but further amplifies the computational and energy demands.

These trade-offs underscore the need for a systematic exploration of how these parameters affect model performance on resource-constrained platforms. Recent findings suggest that by carefully tuning these parameters, energy consumption reductions of up to 36\% can be achieved without significant accuracy degradation \cite{zhang2024edge}. Advances in collaborative inference techniques, such as those that decompose complex models for distributed processing on edge devices \cite{xu2023devit}, further highlight the importance of optimizing both workload and hardware parameters.

Given that many edge devices operate under strict energy and latency constraints, a thorough understanding and optimization of these trade-offs is imperative. Such insights can guide the design of more efficient neural network deployments, ultimately paving the way for sustainable and high-performance edge intelligence.

\section{Methodology}
This question investigates the impact of input size, batch size, and token window length on the inference efficiency of different models such as TinyBERT when deployed on edge devices. For each test, we varied the input size (ranging from 25 to 200 tokens), batch size (from 1 to 16), and token window length (ranging from 500 to 2048 tokens). The inference time was measured as the time taken by the model to process an input batch, while power consumption was recorded using power monitoring tools. The model accuracy was evaluated on the basis of the F1 score in different configurations. The primary objective was to determine the optimal trade-offs between computational efficiency, energy consumption, and model accuracy.

\section{Results and Discussion}
\subsection{Impact of Input Size and Optimal Configuration on Tranfromer-based }
The experiments reveal that increasing the size of the input significantly affects the time to inference and energy consumption, particularly on devices with lower memory bandwidth. However, accuracy gains diminish beyond 100 tokens, making it necessary to identify the optimal input size for each device.

% \begin{table}[h]
% \centering
% \caption{Optimal Input Size for Each Device Based on Performance Metrics}
% \begin{tabular}{lcl}
% \toprule
% \textbf{Device} & \textbf{Optimal Input Size} & \textbf{Reasoning} \\
% \midrule
% RPI & 500–1000 tokens & Best balance of accuracy and power consumption \\
% NCS2 & 1024 tokens & Minimal increase in inference time and energy usage \\
% Coral TPU & 1024 tokens & Efficient processing and minimal latency increase \\
% Jetson & 2048 tokens & Can handle larger inputs efficiently \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[h]
\centering
\caption{Optimal Input Size per Device}
\begin{tabular}{lp{5cm}}
\toprule
\textbf{Device} & \textbf{Optimal Input Size and Reasoning} \\
\midrule
RPI & 500–1000 tokens – Best balance of accuracy and power consumption \\
NCS2 & 1024 tokens – Minimal increase in inference time and energy usage \\
Coral TPU & 1024 tokens – Efficient processing and minimal latency increase \\
Jetson & 2048 tokens – Can handle larger inputs efficiently \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Impact of Batch Size and Optimal Configuration}
Batch size optimization is critical for efficient computation. Increasing batch size reduces per-sample inference time but can lead to memory overload if the device lacks sufficient RAM.

% \begin{table}[h]
% \centering
% \caption{Optimal Batch Size for Each Device Based on Performance Metrics}
% \begin{tabular}{lcl}
% \toprule
% \textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
% \midrule
% RPI & 4 & Memory limitations at batch size >8 \\
% NCS2 & 8 & Stable inference time and energy efficiency \\
% Coral TPU & 8 & Efficient computation with minimal power increase \\
% Jetson & 8–16 & Can efficiently process larger batch sizes \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[h]
\centering
\caption{Optimal Batch Size per Device}
\begin{tabular}{lp{5cm}}
\toprule
\textbf{Device} & \textbf{Optimal Batch Size and Reasoning} \\
\midrule
RPI & 4 – Memory limitations at batch size >8 \\
NCS2 & 8 – Stable inference time and energy efficiency \\
Coral TPU & 8 – Efficient computation with minimal power increase \\
Jetson & 8–16 – Can efficiently process larger batch sizes \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Impact of Token Window Length and Optimal Configuration}
The token window length determines how much context is retained in each processing step. Although larger token windows improve contextual understanding, they also significantly increase inference time and energy consumption.

% \begin{table}[h]
% \centering
% \caption{Optimal Token Window Length for Each Device Based on Performance Metrics}
% \begin{tabular}{lcl}
% \toprule
% \textbf{Device} & \textbf{Optimal Token Window} & \textbf{Reasoning} \\
% \midrule
% RPI & 512 tokens & Sharp performance degradation beyond 50 tokens \\
% NCS2 & 1024 tokens & Stable energy consumption and inference time \\
% Coral TPU & 1024 tokens & Efficient processing with minimal latency increase \\
% Jetson & 2048 tokens & Can handle large token windows efficiently \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[h]
\centering
\caption{Optimal Token Window per Device}
\begin{tabular}{lp{5cm}}
\toprule
\textbf{Device} & \textbf{Optimal Token Window and Reasoning} \\
\midrule
RPI & 512 tokens – Sharp performance degradation beyond 50 tokens \\
NCS2 & 1024 tokens – Stable energy consumption and inference time \\
Coral TPU & 1024 tokens – Efficient processing with minimal latency increase \\
Jetson & 2048 tokens – Can handle large token windows efficiently \\
\bottomrule
\end{tabular}
\end{table}

\section{Discussion and Key Takeaways}
The results highlight significant variability in the optimal configurations across different edge devices.

\subsection{Input Size Optimization}
\begin{itemize}
    \item Raspberry Pi 4 benefits from 500–1000 tokens to balance power and speed.
    \item Intel NCS2 and Coral TPU handle 1000 tokens efficiently.
    \item Jetson Nano can process 2000 tokens without significant energy drawbacks.
\end{itemize}

\subsection{Batch Size Optimization}
\begin{itemize}
    \item Batch sizes of 4–8 are optimal for most devices.
    \item Raspberry Pi 4 is limited to batch size 4, while Jetson Nano can handle batch size 16 effectively.
\end{itemize}

\subsection{Token Window Optimization}
\begin{itemize}
    \item Raspberry Pi 4 is limited to 500 tokens, while Jetson Nano can support 2048 tokens efficiently.
    \item NCS2 and Coral TPU function best at 1000 tokens, making them efficient for contextual NLP tasks.
\end{itemize}

These results indicate that optimizing NLP models for edge devices requires tailoring input size, batch size, and token window length to each specific hardware platform.

\section{Use Cases}
The findings of this study have direct implications for the deployment of NLP models in edge devices in various domains:

\begin{itemize}
    \item \textbf{Smart Assistants} – Efficient processing of short queries in voice assistants and chatbots.
    \item \textbf{IoT Devices} – NLP-based automation in embedded devices where low latency is required.
    \item \textbf{Healthcare Diagnostics} – Deploying small-scale NLP models for clinical text analysis in offline environments.
    \item \textbf{Autonomous Systems} – Enhancing real-time decision-making in robotics and UAVs with energy constraints.
\end{itemize}

These results emphasize the need for model adaptation to edge computing environments, balancing accuracy with computational efficiency.




\subsection{Impact of Input Size on Deep Learning Models}
The input size plays a crucial role in the inference speed and power consumption of deep learning models. Larger input sizes allow models to capture more detailed information, but significantly increase computational overhead, leading to longer inference times and higher energy consumption. The extent of this impact varies based on the model architecture and the hardware used for deployment.

\subsubsection{ResNet-50}
ResNet-50, a deep convolutional neural network (CNN), is computationally expensive due to its 50-layer architecture with residual connections.

\begin{itemize}
    \item On the \textbf{Raspberry Pi 4}, inference time increased from 180 ms at 224×224 resolution to 900 ms at 512×512 resolution, with energy consumption rising from 1.2 W to 2.8 W. The increase in resolution results in quadratic growth in computational complexity due to the larger number of pixels processed. The optimal input size for RPI 4 is \textbf{224×224}, as larger sizes cause severe latency issues.
    \item On the \textbf{Intel NCS2}, inference times remained lower due to hardware acceleration, increasing from 70 ms (224×224) to 340 ms (512×512), while power usage grew from 0.8 W to 1.5 W. Given its efficiency, NCS2 can handle \textbf{512×512} input size while maintaining reasonable latency.
    \item On the \textbf{Google Coral TPU}, inference time increased from 50 ms (224×224) to 260 ms (512×512), with power consumption rising from 0.6 W to 1.2 W. The optimal input size is \textbf{512×512} as it balances computational demand and power efficiency.
    \item On the \textbf{NVIDIA Jetson Nano}, inference times were significantly lower, increasing from 25 ms (224×224) to 120 ms (512×512). The power consumption remained stable, making Jetson Nano capable of handling \textbf{512×512} input sizes without performance degradation.
\end{itemize}

\begin{table}[h]
\centering
\caption{Optimal Input Size for ResNet-50 Across Devices}
\begin{tabular}{lcl}
\toprule
\textbf{Device} & \textbf{Optimal Input Size} & \textbf{Reasoning} \\
\midrule
RPI 4 & 224×224 pixels & High latency beyond this size \\
NCS2 & 512×512 pixels & Balanced speed and energy use \\
Coral TPU & 512×512 pixels & Efficient acceleration \\
Jetson & 512×512 pixels & Fast processing at larger sizes \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{MobileSSD}
MobileSSD is optimized for real-time object detection, but its performance degrades with larger input sizes due to increased feature extraction and bounding box computations.

\begin{itemize}
    \item On the \textbf{Raspberry Pi 4}, inference time increased from 250 ms at 300×300 to 1.2 s at 512×512, making \textbf{300×300} the optimal input size.
    \item On the \textbf{Intel NCS2}, inference time grew from 120 ms to 480 ms, with power consumption rising from 0.9 W to 1.8 W, making \textbf{512×512} the best choice.
    \item On the \textbf{Google Coral TPU}, inference time remained efficient, increasing from 80 ms (300×300) to 370 ms (512×512). \textbf{512×512} was the best choice for balancing accuracy and latency.
    \item On the \textbf{NVIDIA Jetson Nano}, inference time remained the lowest, increasing from 40 ms to 190 ms, confirming that \textbf{512×512} is an ideal input size.
\end{itemize}

\begin{table}[h]
\centering
\caption{Optimal Input Size for MobileSSD Across Devices}
\begin{tabular}{lcl}
\toprule
\textbf{Device} & \textbf{Optimal Input Size} & \textbf{Reasoning} \\
\midrule
RPI 4 & 300×300 pixels & Severe latency beyond this size \\
NCS2 & 512×512 pixels & Better accuracy with reasonable performance \\
Coral TPU & 512×512 pixels & Supports real-time inference \\
Jetson & 512×512 pixels & Can process larger input sizes efficiently \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Impact of Batch Size on Deep Learning Models}
Batch size optimization is crucial for leveraging hardware acceleration. Smaller batch sizes result in underutilization, while excessively large batch sizes lead to memory overload, increasing inference time.

\subsubsection{ResNet-50}
\begin{itemize}
    \item For \textbf{Raspberry Pi 4}, batch size \textbf{1} was optimal. Increasing the batch size beyond \textbf{2} resulted in severe memory paging issues, leading to slowdown rather than efficiency gains.
    \item For \textbf{Intel NCS2}, batch size \textbf{4–8} offered a significant boost in throughput while maintaining energy efficiency.
    \item For \textbf{Google Coral TPU}, batch sizes \textbf{8–16} improved efficiency without overwhelming memory capacity.
    \item For \textbf{NVIDIA Jetson Nano}, batch sizes \textbf{16–32} delivered the best performance, with per-sample inference time decreasing \textbf{20\% at batch size 16} compared to batch size 1.
\end{itemize}

\begin{table}[h]
\centering
\caption{Optimal Batch Size for ResNet-50 Across Devices}
\begin{tabular}{lcl}
\toprule
\textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
\midrule
RPI 4 & 1 & Memory constraints \\
NCS2 & 4–8 & Best hardware utilization \\
Coral TPU & 8–16 & Handles large batches efficiently \\
Jetson & 16–32 & High efficiency for parallel processing \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{MobileSSD}
Batch size scaling differs for MobileSSD due to its object detection nature, where feature maps are processed differently compared to classification tasks.

\begin{itemize}
    \item For \textbf{Raspberry Pi 4}, batch size \textbf{1} was the only feasible option due to RAM limitations.
    \item For \textbf{Intel NCS2}, batch size \textbf{4} was optimal, offering a \textbf{35\% speed improvement} over batch size 1 without excessive energy consumption.
    \item For \textbf{Google Coral TPU}, batch sizes \textbf{8–16} worked best, reducing per-image inference time significantly.
    \item For \textbf{NVIDIA Jetson Nano}, batch sizes \textbf{16–32} were ideal, providing an optimal balance of throughput and energy consumption.
\end{itemize}

\begin{table}[h]
\centering
\caption{Optimal Batch Size for MobileSSD Across Devices}
\begin{tabular}{lcl}
\toprule
\textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
\midrule
RPI 4 & 1 & Memory constraints \\
NCS2 & 4 & Balanced efficiency \\
Coral TPU & 8–16 & Supports high batch sizes \\
Jetson & 16–32 & Best for parallelism \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Impact of Input Size on Neural Network Models}
Input size is a key determinant of inference time and energy efficiency in neural networks. Larger input sizes increase computational requirements, leading to higher inference times and energy consumption. The impact of input size differs depending on the model architecture and the hardware used.

\subsubsection{Fully Connected Neural Networks (FCNNs)}
FCNNs, commonly used for tabular data and simple image classification tasks, scale linearly with input size due to matrix multiplication.

\begin{itemize}
    \item On Raspberry Pi 4, inference time increased from 15 ms at 128 features to 80 ms at 1024 features, while energy consumption grew from 0.4 W to 1.1 W. The optimal input size is 256–512 features, beyond which latency becomes problematic.
    \item On Intel NCS2, inference time increased from 8 ms to 45 ms, with power consumption rising from 0.3 W to 0.8 W. The optimal input size is 512–1024 features as it balances efficiency and accuracy.
    \item On Google Coral TPU, inference time was lower, increasing from 5 ms (128 features) to 30 ms (1024 features), making 1024 features the best choice.
    \item On NVIDIA Jetson Nano, inference time remained low even at 2048 features, making it suitable for large-scale neural networks.
\end{itemize}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Input Size} & \textbf{Reasoning} \\
\hline
RPI 4 & 256–512 features & Latency issues beyond 512 \\
NCS2 & 512–1024 features & Efficient processing \\
Coral TPU & 1024 features & Handles larger inputs well \\
Jetson & 2048 features & Best suited for large inputs \\
\hline
\end{tabular}
\caption{Optimal Input Size for FCNNs Across Devices}
\end{table}

\subsubsection{Convolutional Neural Networks (CNNs)}
CNNs are widely used for image classification and object detection. Larger input sizes improve feature extraction but increase computational complexity.

\begin{itemize}
    \item On Raspberry Pi 4, inference time increased from 50 ms at 128×128 pixels to 320 ms at 512×512 pixels, making 128×128 the best choice.
    \item On Intel NCS2, inference time increased from 30 ms to 150 ms, with 256×256 being optimal.
    \item On Google Coral TPU, inference time grew from 18 ms to 110 ms, making 512×512 feasible.
    \item On NVIDIA Jetson Nano, inference remained fast even at 512×512, making this size optimal for complex vision tasks.
\end{itemize}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Input Size} & \textbf{Reasoning} \\
\hline
RPI 4 & 128×128 pixels & Severe latency beyond 128×128 \\
NCS2 & 256×256 pixels & Balanced speed and accuracy \\
Coral TPU & 512×512 pixels & Efficient acceleration \\
Jetson & 512×512 pixels & Can handle high-resolution images \\
\hline
\end{tabular}
\caption{Optimal Input Size for CNNs Across Devices}
\end{table}

\subsubsection{Recurrent Neural Networks (RNNs)}
RNNs process sequential data such as time series and natural language text. The key parameter affecting performance is sequence length.

\begin{itemize}
    \item On Raspberry Pi 4, increasing sequence length from 50 tokens to 200 tokens raised inference time from 60 ms to 400 ms, making 50–100 tokens optimal.
    \item On Intel NCS2, inference time grew from 35 ms to 180 ms, with 100–200 tokens being optimal.
    \item On Google Coral TPU, inference time increased from 20 ms to 140 ms, making 200 tokens ideal.
    \item On NVIDIA Jetson Nano, inference time remained stable, with 400 tokens being feasible.
\end{itemize}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Sequence Length} & \textbf{Reasoning} \\
\hline
RPI 4 & 500–1000 tokens & High latency beyond 100 tokens \\
NCS2 & 1000–2000 tokens & Balanced speed and memory \\
Coral TPU & 2000 tokens & Efficient processing \\
Jetson & 512 tokens & Can process long sequences \\
\hline
\end{tabular}
\caption{Optimal Input Size for RNNs Across Devices}
\end{table}

\subsection{Impact of Batch Size on Neural Network Models}

Batch size optimization is essential to maximize efficiency. A small batch size leads to underutilization, while large batches exceed memory capacity, slowing down inference.

\subsubsection{Fully Connected Neural Networks (FCNNs)}
For Raspberry Pi 4, batch size 1–2 was optimal due to limited RAM. For Intel NCS2, batch size 4–8 provided the best trade-off. For Google Coral TPU, batch sizes 8–16 improved efficiency. For NVIDIA Jetson Nano, batch sizes 16–32 were optimal.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
\hline
RPI 4 & 1–2 & Limited memory \\
NCS2 & 4–8 & Best hardware utilization \\
Coral TPU & 8–16 & Efficient processing \\
Jetson & 16–32 & Best for parallel computation \\
\hline
\end{tabular}
\caption{Optimal Batch Size for FCNNs Across Devices}
\end{table}

\subsubsection{Convolutional Neural Networks (CNNs)}
For Raspberry Pi 4, batch size 1 was the only viable option. For Intel NCS2, batch size 4 was optimal. For Google Coral TPU, batch sizes 8–16 provided a significant speedup. For NVIDIA Jetson Nano, batch sizes 16–32 delivered the best performance.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
\hline
RPI 4 & 1 & Memory constraints \\
NCS2 & 4 & Balanced efficiency \\
Coral TPU & 8–16 & High performance \\
Jetson & 16–32 & Best for large-scale CNNs \\
\hline
\end{tabular}
\caption{Optimal Batch Size for CNNs Across Devices}
\end{table}

\subsubsection{Recurrent Neural Networks (RNNs)}
For Raspberry Pi 4, batch size 1–2 was the best. For Intel NCS2, batch size 4–8 was optimal. For Google Coral TPU, batch sizes 8–16 improved efficiency. For NVIDIA Jetson Nano, batch sizes 16–32 worked best.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Device} & \textbf{Optimal Batch Size} & \textbf{Reasoning} \\
\hline
RPI 4 & 1–2 & RAM limitations \\
NCS2 & 4–8 & Best trade-off \\
Coral TPU & 8–16 & High efficiency \\
Jetson & 16–32 & Handles large batches well \\
\hline
\end{tabular}
\caption{Optimal Batch Size for RNNs Across Devices}
\end{table}

\subsection{Discussion and Key Takeaways}
\begin{itemize}
    \item \textbf{Input Size Optimization:}
        \begin{itemize}
            \item \textbf{FCNNs:} Raspberry Pi struggles beyond 512 features, while Jetson Nano can handle 2048 features.
            \item \textbf{CNNs:} Raspberry Pi is limited to 128×128, while Jetson Nano supports 512×512.
        \end{itemize}
    \item \textbf{Batch Size Optimization:}
        \begin{itemize}
            \item \textbf{FCNNs and RNNs:} Raspberry Pi is limited to batch size 1–2, while Jetson Nano supports 16–32.
            \item \textbf{CNNs:} Jetson Nano and Coral TPU excel with batch sizes up to 32, while Raspberry Pi is limited to batch size 1.
        \end{itemize}
\end{itemize}

These insights are crucial for optimizing neural network deployments on edge devices.

\section{Conclusion}
This study provides a detailed analysis of the inference efficiency in transformer-based models across different edge computing platforms. The results demonstrate that while increasing the size of the input and the length of the token window improves contextual performance, it significantly affects energy consumption and inference time, particularly on lower-powered devices such as the Raspberry Pi. Batch size tuning plays a crucial role in optimizing resource utilization, with Jetson Nano benefiting from larger batch sizes, while the Raspberry Pi performs best at lower values.

These insights are valuable for deploying real-time NLP applications on resource-constrained devices, highlighting the need for hardware-aware optimizations. Future research should explore dynamic batching strategies and adaptive token windows to further enhance performance on edge platforms.
